An Information Bottleneck Approach for Controlling Conciseness in Rationale Extraction

Decisions of complex language understanding models can be rationalized by limiting their inputs to a relevant subsequence of the original text. A rationale should be as concise as possible without significantly degrading task performance, but this balance can be difficult to achieve in practice. In this paper, we show that it is possible to better manage this trade-off by optimizing a bound on the Information Bottleneck (IB) objective. Our fully unsupervised approach jointly learns an explainer that predicts sparse binary masks over sentences, and an end-task predictor that considers only the extracted rationale. Using IB, we derive a learning objective that allows direct control of mask sparsity levels through a tunable sparse prior. Experiments on ERASER benchmark tasks demonstrate significant gains over norm-minimization techniques for both task performance and agreement with human rationales. Furthermore, we find that in the semi-supervised setting, a modest amount of gold rationales (25% of training examples) closes the gap with a model that uses the full input.

==> sections/bastings.tex <==
\citet{bastings2019interpretable} compare against the best-known previous work on norm regularization \citet{lei2016rationalizing} by making three significant changes: a) Rectifying the latent boolean variables to be exactly 0 or 1 b) exploring a bimodal distribution - Kumaraswamy to replace Bernoulli distribution c) Using lagrangian constraint optimization from \citet{rezende2018taming} by adjusting the lagrangian multiplier $\lambda$ to ensure that the constraint $||m|| - \pi > 0$ is satisfied. While they do not explicitely measure the effect of each of these choices, we explore each of these choices in isolation here, and also investigate their bearings on our sparse prior objective.

\paragraph{Rectified Random Variables}
\citet{louizos2017learning} propose an alternative distribution (Hard Binary) that is reparameterized by once again drawing samples from Uniform $e_j \sim \mathcal{U}(0,1)$ and stretching its support by rectifying its value to lie in $(0 - l_0, 1 + l_1)$ and enforcing $m_j^*$ to be exactly 0 or 1 while still being differentiable.
% rephrase this
$$h = \sigma \left(\frac{\log{p(m_j|x)} + g_j}{\tau}\right)$$
$$h' = h(l_1-l_0) + l_0$$
$$m_j^* = \min{(1, \max{(0, h')})}$$
% \citet{bastings2019interpretable} use this technique to minimize the expected value of the L0 norm of $m$.
This is a much stricter training regimen as entire sentences are completely zeroed-out and disregarded even during training.
This choice allows them to optimize explicitely for the expected value of the L0 norm, $||m||_0$ by sampling $m_j$ from a Hard Binary distribution \cite{louizos2017learning}. Specifically, $L_0 = ||m||_0$ can be estimated as :
$$L_0 = \sum_{j} \sigma(\log{p(m_j|x)} - \tau \log{\frac{-l_0}{l_1}})$$
% that can be reparameterized \cite{kingma2015variational}.
% $$L = \mathbf{E}_{m \sim p(m|x)}[-\log{q(y|z)] + \gamma ||m_j||_0$$
Our empirical results reflect that the concrete binary distribution produces the same results as the reparameterized Bernoulli distribution. 

\paragraph{Kumaraswamy Distribution}
\label{kuma}
\cite{bastings2019interpretable} further replace the rectified Hard Binary with a recitified Kumaraswamy distribution. It is possible to adopt this distribution even for our sparse-prior objective. The KL divergence between the Kumaraswamy and Beta distribution can be computed, as done in this work \cite{nalisnick2017stick}.

% \paragraph{Lagrangian Constraint Optimization}
% \cite{bastings2019interpretable} also propose using variable Lagrangian multipliers for the constraint $||m|| - \pi > 0$, by adopting the technique proposed in  \cite{rezende2018taming}. We find that the KL divergence based optimization can guarantee desired sparsity in the mask without adding further complexity to the optimization.
